Bridging Dictionary: AI-Generated Dictionary of Partisan Language Use

Words often carry different meanings for people from diverse backgrounds. Today's era of social polarization demands that we choose words carefully to prevent miscommunication, especially in political communication and journalism. To address this issue, we introduce the Bridging Dictionary, an interactive tool designed to illuminate how words are perceived by people with different political views. The Bridging Dictionary includes a static, printable document featuring 796 terms with summaries generated by a large language model. These summaries highlight how the terms are used distinctively by Republicans and Democrats. Additionally, the Bridging Dictionary offers an interactive interface that lets users explore selected words, visualizing their frequency, sentiment, summaries, and examples across political divides. We present a use case for journalists and emphasize the importance of human agency and trust in further enhancing this tool. The deployed version of Bridging Dictionary is available at https://dictionary.ccc-mit.org/.

==> figures/channel-topic-table.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{images/channel-topic-table.png}
    \caption{The topics detected in channel-wide comments.}
    \label{fig:channel-topic-table}
\end{wrapfigure}

==> figures/channel-video.tex <==
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/video-dashboard-view.png}
        \Description{An example of the dashboard view shown for each video.}
        \caption{An example of the dashboard view shown for each video.}
        \label{fig:video-dashboard-view}
    \end{subfigure}
    \hfill % no blank lines here!
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/channel-themes.png}
        \Description{GPT-generated themes at the channel level.}
        \caption{GPT-generated themes at the channel level.}
        \label{fig:channel-themes}
    \end{subfigure}
    \Description{Selected views of the app interface: a video-level dashboard of comments, and channel-level generated themes.}
    \caption{Selected views of the app interface: a video-level dashboard of comments, and channel-level generated themes.}
    \label{fig:interface}
\end{figure}
